Exponential Quantum One-Wayness and EFI Pairs

In classical cryptography, one-way functions are widely considered to be the minimal computational assumption. However, when taking quantum information into account, the situation is more nuanced. There are currently two major candidates for the minimal assumption: the search quantum generalization of one-way functions are one-way state generators (OWSG), whereas the decisional variant are EFI pairs. A well-known open problem in quantum cryptography is to understand how these two primitives are related. A recent breakthrough result of Khurana and Tomer (STOC'24) shows that OWSGs imply EFI pairs, for the restricted case of pure states. In this work, we make progress towards understanding the general case. To this end, we define the notion of inefficiently-verifiable one-way state generators (IV-OWSGs), where the verification algorithm is not required to be efficient, and show that these are precisely equivalent to EFI pairs, with an exponential loss in the reduction. Significantly, this equivalence holds also for mixed states. Thus our work establishes the following relations among these fundamental primitives of quantum cryptography: (mixed) OWSGs => (mixed) IV-OWSGs $\equiv_{\rm exp}$ EFI pairs, where $\equiv_{\rm exp}$ denotes equivalence up to exponential security of the primitives.

==> EFI_from_OWSG_backup.tex <==
\section{EFI from exponentially-secure mixed OWSGs}

\begin{definition}[OWSGs]
A OWSG is a pair $(\StateGen,\Ver)$ of algorithms such that
\begin{itemize}
    \item 
    $\StateGen(k)\to\phi_k:$
    It is a QPT algorithm that, on input $k\in\bit^\secp$, outputs an $n$-qubit state $\phi_k$.
    \item 
    $\Ver(k',\phi_k)\to\bot/\top:$
    It is a QPT algorithm that, on input $k'$ and $\phi_k$, outputs $\top/\bot$.
\end{itemize}
\end{definition}

\begin{definition}[Exponential security of OWSGs]
We say that a OWSG is $\delta$ exponentially secure if for any QPT adversary $\cA$ and any polynomial $t$,
\begin{align}
\Pr[\top\gets\Ver(k',\phi_k):k\gets\bit^\secp,\phi_k^{\otimes t}\gets\StateGen(k)^{\otimes t},k'\gets\cA(1^\secp,\phi_k^{\otimes t})]    
\le 2^{-\delta}.
\end{align}
\end{definition}



\begin{lemma}
Let $p$ be any polynomial, and
define
\begin{align}
G_k\coloneqq \left\{k'\in\bit^\secp:\Pr[\top\gets\Ver(k',\phi_k)]\ge 1-\frac{1}{p(\secp)}\right\}.    
\end{align}
Let $r$ be a positive real number such that 
$\delta+r \ge c\secp$ with a constant $c>1$.
Then, except for a negligible fraction of $k\in\bit^\secp$, $|G_k|\le 2^r$.
\end{lemma}
\begin{proof}
Let us consider the following trivial attack to the OWSG: given $\phi_k^{\otimes t}$, just ignore it, sample $k'\gets\bit^\secp$, and output $k'$.
Due to the $\delta$ exponential security of the OWSG, the winning probability of the trivial attack should be at most $2^{-\delta}$:
\begin{align}
\frac{1}{2^{2\secp}}\sum_{k,k'\in\bit^\secp} \Pr[\top\gets\Ver(k',\phi_k)]\le2^{-\delta}.
\end{align}
Let us define the set
\begin{align}
T\coloneqq\{k\in\bit^\secp:|G_k|\ge 2^r\}.    
\end{align}
Then,
\begin{align}
2^{-\delta}
&\ge\frac{1}{2^{2\secp}}\sum_{k,k'\in\bit^\secp} \Pr[\top\gets\Ver(k',\phi_k)]\\
&\ge\frac{1}{2^{2\secp}}\sum_{k\in\bit^\secp} 
\sum_{k'\in G_k}\Pr[\top\gets\Ver(k',\phi_k)]\\
&\ge\frac{1-\frac{1}{p}}{2^{2\secp}}\sum_{k\in\bit^\secp}|G_k|\\
&\ge\frac{1-\frac{1}{p}}{2^{2\secp}}\sum_{k\in T}|G_k|\\
&\ge\frac{(1-\frac{1}{p})2^r|T|}{2^{2\secp}}.
\end{align}
It means that
\begin{align}
\frac{|T|}{2^\secp}
\le\frac{2^\secp}{2^{\delta+r}(1-\frac{1}{p})}
\le\negl(\secp)
\end{align}
if $\delta+r \ge c\secp$ with $c>1$.
\end{proof}




\begin{theorem}
Let $\delta\ge (0.5+d)\secp$, where $d>0$ is any constant. 
If $\delta$-exponentially-secure OWSGs exist, then EFI pairs exist.    
\end{theorem}

\begin{proof}
Let $0<\epsilon<1$ be a small constant.
Let $r\coloneqq(0.5+\frac{d}{2})\secp$.
Let $\eta$ be the smallest integer such that $(1+\epsilon)^\eta\ge 2^{r+1}$.
Let $\cH_{\secp,j}\coloneqq\{h:\cX\to\cY\}$ be the family of pairwise independent hash functions such that
$\cX\coloneqq\bit^\secp$ and $\cY\coloneqq[M_j]$, where
$M_j\coloneqq \lceil (1+\epsilon)^j\rceil$.
We define the following two states that are used for the commitment of 0 and 1, respectively.
\begin{align}
\ket{\psi_{0,\secp}}_{\regR,\regC}&\coloneqq
\frac{1}{\sqrt{2^\secp}}
\sum_{k\in\bit^\secp}
\frac{1}{\sqrt{\eta}}
\sum_{j\in\{0,1,...,\eta-1\}}
\frac{1}{\sqrt{|\cH_{\secp,j}|}}
\sum_{h\in\cH_{\secp,j}}   
\ket{k,j,h}_{\regC_1}\ket{j,h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\\
\ket{\psi_{1,\secp}}_{\regR,\regC}&\coloneqq
\frac{1}{\sqrt{2^\secp}}
\sum_{k\in\bit^\secp}
\frac{1}{\sqrt{\eta}}
\sum_{j\in\{0,1,...,\eta-1\}}
\frac{1}{\sqrt{|{\mathcal H_{\secp,j}}|}}
\sum_{h\in\cH_{\secp,j}}   
\ket{k,j,h}_{\regC_1}\ket{j,h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{k}_{\regR_3}.
\end{align}
Here, $\regR\coloneqq(\regR_1,\regR_2,\regR_3)$ and $\regC\coloneqq(\regC_1,\regC_2)$.
Without loss of generality, we can assume that $\StateGen$ runs as follows:
generate a pure state
$\ket{\Phi_k}_{\regA,\regB}$ and output the register $\regA$.
Then, we have $\phi_k=\Tr_{\regB}(\ket{\Phi_k}_{\regA,\regB})$.
We define $\regC_2\coloneqq (\regB_1,...,\regB_t)$
and
$\regR_2\coloneqq (\regA_1,...,\regA_t)$.
It is clear that both $\ket{\psi_{0,\secp}}$ and $\ket{\psi_{1,\secp}}$ are efficiently generatable.
For the notational simplicity, in the following we omit $\secp$ of $\ket{\psi_{b,\secp}}$ and $\cH_{\secp,j}$.



\paragraph{Computational binding.}
First we show the computational binding.
For the sake of contradiction, we assume that our construction does not satisfy the computational binding.
It means that there exists a polynomial $q$, a quantum advice state $\ket{\tau}_\regZ$ on the register $\regZ$, and
a QPT unitary $U$ acting on $\regR$ and $\regZ$ such that
\begin{align}
\|\bra{\psi_1}_{\regC,\regR}(I_\regC\otimes U_{\regR,\regZ})(\ket{\psi_0}_{\regC,\regR}\ket{\tau}_\regZ)\|^2\ge\frac{1}{q(\secp)}
\end{align}
for infinitely-many $\secp$.
This means that
\begin{align}
\frac{1}{q(\secp)}
&\le\left\|
\sum_{k,j,h}\frac{1}{2^\secp\eta|\cH_{j}|} 
\bra{j,h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
(I_{\regC_3}\otimes U_{\regR,\regZ})
\ket{j,h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
&\le\left(\sum_{k,j,h}\frac{1}{2^\secp\eta|\cH_{j}|} 
\left\|\bra{j,h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
(I_{\regC_3}\otimes U_{\regR,\regZ})
\ket{j,h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|\right)^2\\
&\le\sum_{k,j,h}\frac{1}{2^\secp\eta|\cH_{j}|} 
\left\|\bra{j,h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
(I_{\regC_3}\otimes U_{\regR,\regZ})
\ket{j,h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
&\le\sum_{k,j,h}\frac{1}{2^\secp\eta|\cH_{j}|}
\left\|\bra{k}_{\regR_3}
(I_{\regC_3}\otimes U_{\regR,\regZ})
\ket{j,h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\label{last}.
\end{align}

From such $\ket{\tau}$ and $U$, we can construct an adversary $\cA$ that breaks the security of the OWSG as follows:
\begin{enumerate}
    \item 
    Get the $\regR_2$ register of $\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}$ and $\ket{\tau}_\regZ$ as input.
    \item 
    Choose $j\gets\{0,1,...,\eta-1\}$ and $h\gets\cH_{j}$. Choose $y\gets [M_j]$.
    \item 
    Apply $I_{\regC_3}\otimes U_{\regR,\regZ}$ on $\ket{j,h,y}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ$.
    \item
    Measure the register $\regR_3$ in the computational basis, and output the result.
\end{enumerate}
The probability that $\cA$ outputs $k$ is 
\begin{align}
&\sum_{k,j,h}\frac{1}{2^\secp\eta|\cH_{j}|}
\sum_{y\in [M_j]}\frac{1}{M_j}
\left\|\bra{k}_{\regR_3}
(I_{\regC_3}\otimes U_{\regR,\regZ})
\ket{j,h,y}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
&\ge
\sum_{k,j,h}\frac{1}{2^\secp\eta|\cH_{j}|}
\frac{1}{2^{r+1}}
\left\|\bra{k}_{\regR_3}
(I_{\regC_3}\otimes U_{\regR,\regZ})
\ket{j,h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
&\ge\frac{1}{2^{r+1}q}.
\end{align}
Because
\begin{align}
\frac{1}{2^{r+1}q}-\frac{1}{2^\delta}
=\frac{2^\delta-2^{r+1}q}{2^{r+1+\delta}q}
\ge\frac{2^{(0.5+d)\secp}-2^{(0.5+d/2)\secp+1}2^{\frac{d}{4}\secp}}{2^{r+1+\delta}q}>0,
\end{align}
the $\delta$ exponential security of the OWSG is broken.
Hence the computational binding is shown.

\paragraph{Statistical hiding.}
Next we show the statistical hiding.
Let $\cV$ be the following quantum algorithm.
\begin{enumerate}
    \item 
Get $j$, $h$, $h(k)$, and the $\regR_3$ register of $\ket{\Phi_k^{\otimes t}}_{\regR_3,\regC_3}$ as input.
\item 
Do the shadow tomography and construct the list of all $k'\in\bit^\secp$ such that
$\Ver(k',\phi_k)\ge1-\frac{1}{p(\secp)}$.
\item 
Compute $h(k')$ for each $k'$ in the list.
If there is only a single $k^*$ in the list such that $h(k^*)=h(k)$, output $k^*$.
Otherwise, output $\bot$.
\end{enumerate}


For any $k\in\bit^\secp$,
there exists $j^*\in\{0,1,...,\eta-1\}$ such that
$ M_{j^*}
\le 2|G_k|\le
(1+\epsilon)M_{j^*}$.
With probability $\frac{1}{\eta}=\frac{1}{\poly(\secp)}$, such $j^*$ is chosen.
Then for such $j^*$, 
due to the pair-wise independence of $h$,
\begin{align}
\Pr_{h\gets\mathcal{H}_{j^*}}[|G_k\cap h^{-1}(h(k))|=1]
&\ge\frac{|G_k|}{M_{j^*}}-\frac{|G_k|^2}{M_{j^*}^2}    \\
&\ge\frac{1}{2}-\frac{(1+\epsilon)^2}{4}.
\end{align}
Hence there exists a unitary $U_\regR$ such that
\begin{align}
|\bra{\psi_{1}}(I_\regC\otimes U_\regR)\ket{\psi_{0}}|^2    
\ge\frac{1}{\poly(\secp)}.
\end{align}
Due to the Uhlmann's theorem, it means that
$F(\rho_0,\rho_1)\ge\frac{1}{\poly(\secp)}$.
\end{proof}

==> backup2_EFI_from_OWSGs.tex <==
\section{Exponentially-Secure IV-OWSGs Imply EFI pairs}
\label{sec:exp_IVOWSG_EFI}
In this section, we show our main result, namely, the construction of EFI pairs from exponentially-secure IV-OWSGs. 
Before stating our main theorem, we prove a useful lemma below.

\begin{lemma}\label{lem:1}
Let $(\KeyGen,\StateGen,\Ver)$ be a $\delta$-exponentially-secure IV-OWSG. For any polynomial $p=p(\lambda)$ define 
\begin{align*}
G_k\coloneqq \left\{k':\Pr[\top\gets\Ver(k',\phi_k)]\ge 1-\frac{1}{p(\secp)}\right\}.    
\end{align*}
Then 
except for a negligible fraction of $k$,
\begin{align}
1\le |G_k|\le 2^r
\end{align}
for any $r$ such that $\delta+r \ge C\secp$, for some constant $C > 1$.
\end{lemma}
\begin{proof}
$1\le|G_k|$ except for a negligible fraction of $k$ is shown from the correctness of IV-OWSGs.
Let us show that $|G_k|\le2^r$ except for a negligible fraction of $k$.
Consider the following trivial attack against the IV-OWSG: On input $\phi_k^{\otimes t}$, ignore the state, sample $k' \gets \bit^\secp$,
and output $k'$. By the $\delta$-exponential security of the IV-OWSG, the winning probability of the trivial attack should be at most $2^{-\delta}$. In other words:
\begin{align*}
\sum_{k,k'}\Pr[k]2^{-\secp} \Pr[\top\gets\Ver(k',\phi_k)]\le 2^{-\delta},
\end{align*}
where $\Pr[k]\coloneqq\Pr[k\gets\KeyGen(1^\secp)]$.
%\begin{align*}
%\frac{1}{2^{2\secp}}\sum_{k,k'\in\KeyGen(1^\secp)} \Pr[\top\gets\Ver(k',\phi_k)]\le 2^{-\delta}.
%\end{align*}

Let us define the set of keys 
\begin{align*}
T\coloneqq\{k:|G_k|\ge 2^r\}.    
\end{align*}
Then we rewrite
\begin{align*}
2^{-\delta}
&\ge\sum_{k,k'}\Pr[k]2^{-\secp} \Pr[\top\gets\Ver(k',\phi_k)]\\
&\ge\sum_{k\in T}\Pr[k] \sum_{k'\in G_k}2^{-\secp}\Pr[\top\gets\Ver(k',\phi_k)]\\
&\ge\frac{1-\frac{1}{p(\lambda)}}{2^{\secp}}\sum_{k\in T}\Pr[k]|G_k|\\
&\ge\frac{1-\frac{1}{p(\lambda)}}{2^{\secp}}2^r\sum_{k\in T}\Pr[k].
\end{align*}
Putting things together, we obtain that
\begin{align*}
\sum_{k\in T}\Pr[k]
\le\frac{2^\secp}{2^{\delta+r}(1-\frac{1}{p(\lambda)})}
\end{align*}
which is negligible if $\delta+r \ge C\secp$, for some $C>1$.
\end{proof}
We are now ready to show the main theorem of this section.
\begin{theorem}\label{thm:EFI_from_IV-OWSG}
Let $\delta\ge (0.5+D)\secp$, for any constant $D>0$. If $\delta$-exponentially secure IV-OWSGs exist, then EFI pairs exist.    
\end{theorem}
\begin{proof}
Let $r\coloneqq(0.5+\frac{D}{2})\secp$ and let $\cH\coloneqq\{h:\cX\to\cY\}$ be the family of pairwise independent hash functions such that $\cX\coloneqq\bit^\secp$ and $\cY\coloneqq\{1,\dots, 2\lfloor 2^r\rfloor\}$. By \cref{cor:com_to_EFI} it suffices to show that IV-OWSGs imply canonical quantum bit commitment schemes that satisfy statistical $(1-1/\poly(\secp))$-hiding and computational binding. 
Assume that an IV-OWSG $(\KeyGen,\StateGen,\Ver)$ exists.
From it, we construct a bit commitment scheme as follows.
We define the following two states, that we shall think of being the commitments of $0$ and $1$, respectively:
\begin{align}
\ket{\psi_{0}}_{\regR,\regC}&\coloneqq
\sum_{k}
\sum_{h\in\cH}   
\sqrt{\frac{\Pr[k]}{|\cH|}}
\ket{k,junk_k,h}_{\regC_1}\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\\
\ket{\psi_1}_{\regR,\regC}&\coloneqq
\sum_{k}
\sum_{h\in\cH}   
\sqrt{\frac{\Pr[k]}{|\cH|}}
\ket{k,junk_k,h}_{\regC_1}\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{k}_{\regR_3},
\end{align} 
where $\Pr[k]\coloneqq\Pr[k\gets\KeyGen(1^\secp)]$ and $junk$ is the junk state of $\KeyGen$.\footnote{
Without loss of generality, we can assume that $\KeyGen$ algorithm runs as follows.
Generate the state
$\sum_{k}\sqrt{\Pr[k]}|k\rangle|junk_k\rangle$, measure the first register, and output the result.
}
We denote by $\regC\coloneqq(\regC_1,\regC_2)$ the commitment register and by $\regR\coloneqq(\regR_1,\regR_2,\regR_3)$ the opening register.
Without loss of generality, we can assume that $\StateGen$ generates a pure state
$\ket{\Phi_k}_{\regA,\regB}$ and outputs the register $\regA$.
Then, we have $\phi_k=\Tr_{\regB}(\ket{\Phi_k}_{\regA,\regB})$ and consequently we define $\regC_2\coloneqq (\regB_1,...,\regB_t)$
and
$\regR_2\coloneqq (\regA_1,...,\regA_t)$.
It is clear that both $\ket{\psi_0}$ and $\ket{\psi_1}$ are efficiently generatable. 
In the following we show that the scheme is 
statistical $(1-1/\poly(\secp))$-hiding and computational binding.  



\paragraph{Computational binding.}
Towards a contradiction, we assume that our construction does not satisfy the computational binding.
This means that there exists a polynomial $q=q(\lambda)$, a quantum advice state $\ket{\tau}_\regZ$ on the register $\regZ$,  and
a QPT unitary $U$ acting on $\regR$ and $\regZ$ such that
\begin{align*}
\|\bra{\psi_1}_{\regC,\regR}(I_\regC\otimes U_{\regR,\regZ})(\ket{\psi_0}_{\regC,\regR}\ket{\tau}_\regZ)\|^2\ge\frac{1}{q(\secp)}
\end{align*}
for infinitely-many $\secp$. This means that
\begin{align*}
\frac{1}{q(\secp)}
&\le\left\|
\sum_{k,h}\frac{\Pr[k]}{|\cH|} 
\bra{h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
(I_{\regC_2}\otimes U_{\regR,\regZ})
\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
&\le\left(\sum_{k,h}\frac{\Pr[k]}{|\cH|} 
\left\|\bra{h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
(I_{\regC_2}\otimes U_{\regR,\regZ})
\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|\right)^2\\
&\le\sum_{k,h}\frac{\Pr[k]}{|\cH|} 
\left\|\bra{h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
(I_{\regC_2}\otimes U_{\regR,\regZ})
\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
&\le\sum_{k,h}\frac{\Pr[k]}{|\cH|}
\left\|\bra{k}_{\regR_3}
(I_{\regC_2}\otimes U_{\regR,\regZ})
\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\label{last}.
\end{align*}
Here, in the second inequality we have used the triangle inequality, and in the third inequality we have used Jensen's inequality.
From such $\ket{\tau}$ and $U$, we can construct a QPT adversary $\cA$ that breaks the security of the IV-OWSG as follows:
\begin{itemize}
    \item 
    Get the $\regR_2$ register of $\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}$ and $\ket{\tau}_\regZ$ as input.
    \item 
    Choose $h\gets\cH$. Choose $y\gets \cY$.
    \item 
    Apply $(I_{\regC_2}\otimes U_{\regR,\regZ})$ on $\ket{h,y}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ$.
    \item
    Measure the register $\regR_3$ in the computational basis, and output the result.
\end{itemize}
The probability that $\cA$ outputs $k$ is 
\begin{align*}
&\sum_{k,h}\frac{\Pr[k]}{|\cH|}
\sum_{y\in \cY}\frac{1}{|\cY|}
\left\|\bra{k}_{\regR_3}
(I_{\regC_3}\otimes U_{\regR,\regZ})
\ket{h,y}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
&\ge
\sum_{k,h}\frac{\Pr[k]}{|\cH|}
\frac{1}{2\lfloor 2^r\rfloor}
\left\|\bra{k}_{\regR_3}
(I_{\regC_3}\otimes U_{\regR,\regZ})
\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
&\ge\frac{1}{2q(\lambda)\lfloor 2^r\rfloor}.
\end{align*}
Because
\begin{align*}
\frac{1}{2q(\lambda)\lfloor 2^r\rfloor}-\frac{1}{2^\delta}
=\frac{2^\delta-2q(\lambda)\lfloor 2^r\rfloor}{2q(\lambda)2^\delta\lfloor 2^r\rfloor}
\ge\frac{2^\delta-2q(\lambda)2^r}{2q(\lambda)2^\delta\lfloor 2^r\rfloor}>0,
\end{align*}
$\cA$ breaks the one-wayness of the IV-OWSG with probability $>2^{-\delta}$, which is a contradiction.
Thus, the above scheme satisfies computational binding. 

\paragraph{Statistical hiding.} 
Fix any polynomial $p=p(\secp)$.
Consider the following (inefficient) algorithm that can access only the $\regR$ register of $\ket{\psi_0}_{\regR,\regC}$.
\begin{itemize}
\item Apply the shadow tomography procedure (setting $\varepsilon = 1/p(\lambda)$ and $\omega = 2^{-\lambda}$) 
    on $\regR_2$ register of $\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}$
to obtain the list of all $k'$ such that
$\Ver(k',\phi_k)\ge1-\frac{1}{p(\secp)}$.
\item 
Read $(h,h(k))$ from $\regR_1$.
Compute $h(k')$ for each $k'$ in the list.
If there is only a single $k^*$ in the list such that $h(k^*)=h(k)$, output $k^*$.
Otherwise, output $\bot$.
\end{itemize}
By the pairwise independence of $h$ and by \cref{lem:1}, we have that
\begin{align*}
\Pr_{h\gets\cH}[|G_k\cap h^{-1}(h(k))|=1]
\ge1-\frac{|G_k|}{|\cY|}
=1-\frac{|G_k|}{2\lfloor 2^r\rfloor}
\ge\frac{1}{2}
\end{align*}
except for a negligible fraction of $k$.
Setting $t = t(\lambda)$ to be a large enough polynomial, by \cref{lem:ST}, the above inefficient algorithm outputs $k^*$
with probability at least $\frac{1}{2}$.
If we purify the algorithm, we have a unitary $U_\regR$ such that \takashi{Should we introduce an ancilla here? That is, should we write
\begin{align*}
|\bra{\psi_{1}}_{\regR,\regC}(I_\regC\otimes U_{\regR,\regZ})\ket{\psi_{0}}_{\regR,\regC}\ket{0...0}_{\regZ}|^2    
\ge\frac{1}{2}-\negl(\secp)?
\end{align*}
I believe this is sufficient for our purpose. 
It's not immediately clear to me if we can remove the ancilla.
}
\begin{align*}
|\bra{\psi_{1}}_{\regR,\regC}(I_\regC\otimes U_\regR)\ket{\psi_{0}}_{\regR,\regC}|^2    
\ge\frac{1}{2}-\negl(\secp).
\end{align*}
By Uhlmann's theorem we have
\begin{align}
F(\rho_0,\rho_1)\ge\frac{1}{2} - \negl(\lambda)
\end{align}
where $\rho_b\coloneqq\Tr_{\regR}(\ket{\psi_b}_{\regR,\regC})$.
Consequently, $\TD(\rho_0,\rho_1)\le\frac{1}{\sqrt{2}} + \negl(\lambda)$.
This implies that the scheme satisfies 
statistical $(\frac{1}{\sqrt{2}} + \negl(\lambda))$-hiding, which in particular implies that it satisfies statistical $(1-1/\poly(\secp))$-hiding. 
This completes the proof of \Cref{thm:EFI_from_IV-OWSG}. %\takashi{The parallel repetition step is no longer needed since it is already implicitly done in \cref{cor:com_to_EFI}}
\if0
\paragraph{Parallel Repetition.} The above argument shows that there exists a commitment which is computationally binding with negligible probability and $\frac{1}{\sqrt{2}} + \negl(\lambda)$ statistically hiding. The conversion theorem from  \cite{EC:HhaMorYam23} implies that there exists a commitment that is $\negl(\lambda)$ computationally hiding and $\frac{1}{\sqrt{2}} + \negl(\lambda)$ statistically binding. \takashi{I guess there is a quadratic loss in the flavor conversion, and thus this should be $\frac{1}{2^{1/4}} + \negl(\lambda)$ statistically binding. I'll check it and deal with it soon.} By a standard parallel repetition argument, we obtain a commitment which is both statistically binding and computationally hiding with negligible error.
\fi
\end{proof}

%\textcolor{red}{\textbf{GM Marker.}}

% \section{EFI from exponentially-secure mixed OWSGs}
% \takashi{Doesn't this direction work from exponentially-secure IV-OWSGs instead of OWSGs? I don't think the efficient verifiabilility is used in the proof.}
% \begin{definition}[OWSGs] 
% A OWSG is a pair $(\StateGen,\Ver)$ of algorithms such that
% \begin{itemize}
%     \item 
%     $\StateGen(k)\to\phi_k:$
%     It is a QPT algorithm that, on input $k\in\bit^\secp$, outputs an $n$-qubit state $\phi_k$.
%     \item 
%     $\Ver(k',\phi_k)\to\bot/\top:$
%     It is a QPT algorithm that, on input $k'$ and $\phi_k$, outputs $\top/\bot$.
% \end{itemize}
% \end{definition}

% \begin{definition}[Exponential security of OWSGs]
% We say that a OWSG is $\delta$-exponentially-secure if for any QPT adversary $\cA$ and any polynomial $t$,
% \begin{align}
% \Pr[\top\gets\Ver(k',\phi_k):k\gets\bit^\secp,\phi_k^{\otimes t}\gets\StateGen(k)^{\otimes t},k'\gets\cA(1^\secp,\phi_k^{\otimes t})]    
% \le 2^{-\delta}.
% \end{align}
% \end{definition}


% We use the following lemma to show our main result.
% \begin{lemma}
% Let $(\StateGen,\Ver)$ be a $\delta$-exponentially-secure OWSG,  
% $p$ be any polynomial, and
% define
% \begin{align}
% G_k\coloneqq \left\{k'\in\bit^\secp:\Pr[\top\gets\Ver(k',\phi_k)]\ge 1-\frac{1}{p(\secp)}\right\}.    
% \end{align}
% Let $r$ be a polynomial such that
% $\delta+r \ge c\secp$ with a constant $c>1$.
% Then, except for a negligible fraction of $k\in\bit^\secp$, $|G_k|\le 2^r$.
% \end{lemma}
% \begin{proof}
% Let us consider the following trivial attack to the OWSG: given $\phi_k^{\otimes t}$, just ignore it, sample $k'\gets\bit^\secp$, and output $k'$.
% Due to the $\delta$ exponential security of the OWSG, the winning probability of the trivial attack should be at most $2^{-\delta}$:
% \begin{align}
% \frac{1}{2^{2\secp}}\sum_{k,k'\in\bit^\secp} \Pr[\top\gets\Ver(k',\phi_k)]\le2^{-\delta}.
% \end{align}
% Let us define the set
% \begin{align}
% T\coloneqq\{k\in\bit^\secp:|G_k|\ge 2^r\}.    
% \end{align}
% Then,
% \begin{align}
% 2^{-\delta}
% &\ge\frac{1}{2^{2\secp}}\sum_{k,k'\in\bit^\secp} \Pr[\top\gets\Ver(k',\phi_k)]\\
% &\ge\frac{1}{2^{2\secp}}\sum_{k\in\bit^\secp} 
% \sum_{k'\in G_k}\Pr[\top\gets\Ver(k',\phi_k)]\\
% &\ge\frac{1-\frac{1}{p}}{2^{2\secp}}\sum_{k\in\bit^\secp}|G_k|\\
% &\ge\frac{1-\frac{1}{p}}{2^{2\secp}}\sum_{k\in T}|G_k|\\
% &\ge\frac{(1-\frac{1}{p})2^r|T|}{2^{2\secp}}.
% \end{align}
% It means that
% \begin{align}
% \frac{|T|}{2^\secp}
% \le\frac{2^\secp}{2^{\delta+r}(1-\frac{1}{p})}
% \le\negl(\secp)
% \end{align}
% if $\delta+r \ge c\secp$ with $c>1$.
% \end{proof}




% \begin{theorem}
% Let $\delta\ge (0.5+d)\secp$, where $d>0$ is any constant. 
% If $\delta$-exponentially-secure OWSGs exist, then EFI pairs exist.    
% \end{theorem}

% \begin{proof}
% Let $0<\epsilon<1$ be a small constant.
% Let $r\coloneqq(0.5+\frac{d}{2})\secp$.
% Let $\cH\coloneqq\{h:\cX\to\cY\}$ be the family of pairwise independent hash functions such that
% $\cX\coloneqq\bit^\secp$ and $\cY\coloneqq[2\lfloor 2^r\rfloor]$.
% We define the following two states that are used for the commitment of 0 and 1, respectively.
% \begin{align}
% \ket{\psi_{0}}_{\regR,\regC}&\coloneqq
% \frac{1}{\sqrt{2^\secp}}
% \sum_{k\in\bit^\secp}
% \frac{1}{\sqrt{|\cH|}}
% \sum_{h\in\cH}   
% \ket{k,h}_{\regC_1}\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\\
% \ket{\psi_1}_{\regR,\regC}&\coloneqq
% \frac{1}{\sqrt{2^\secp}}
% \sum_{k\in\bit^\secp}
% \frac{1}{\sqrt{|\cH|}}
% \sum_{h\in\cH}   
% \ket{k,h}_{\regC_1}\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{k}_{\regR_3}.
% \end{align}
% Here, $\regR\coloneqq(\regR_1,\regR_2,\regR_3)$ and $\regC\coloneqq(\regC_1,\regC_2)$.
% Without loss of generality, we can assume that $\StateGen$ runs as follows:
% generate a pure state
% $\ket{\Phi_k}_{\regA,\regB}$ and output the register $\regA$.
% Then, we have $\phi_k=\Tr_{\regB}(\ket{\Phi_k}_{\regA,\regB})$.
% We define $\regC_2\coloneqq (\regB_1,...,\regB_t)$
% and
% $\regR_2\coloneqq (\regA_1,...,\regA_t)$.
% It is clear that both $\ket{\psi_0}$ and $\ket{\psi_1}$ are efficiently generatable.



% \paragraph{Computational binding.}
% First we show the computational binding.
% For the sake of contradiction, we assume that our construction does not satisfy the computational binding.
% It means that there exists a polynomial $q$, a quantum advice state $\ket{\tau}_\regZ$ on the register $\regZ$, and
% a QPT unitary $U$ acting on $\regR$ and $\regZ$ such that
% \begin{align}
% \|\bra{\psi_1}_{\regC,\regR}(I_\regC\otimes U_{\regR,\regZ})(\ket{\psi_0}_{\regC,\regR}\ket{\tau}_\regZ)\|^2\ge\frac{1}{q(\secp)}
% \end{align}
% for infinitely-many $\secp$.
% This means that
% \begin{align}
% \frac{1}{q(\secp)}
% &\le\left\|
% \sum_{k,h}\frac{1}{2^\secp|\cH|} 
% \bra{h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
% (I_{\regC_3}\otimes U_{\regR,\regZ})
% \ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
% &\le\left(\sum_{k,h}\frac{1}{2^\secp|\cH|} 
% \left\|\bra{h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
% (I_{\regC_3}\otimes U_{\regR,\regZ})
% \ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|\right)^2\\
% &\le\sum_{k,h}\frac{1}{2^\secp|\cH|} 
% \left\|\bra{h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
% (I_{\regC_3}\otimes U_{\regR,\regZ})
% \ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
% &\le\sum_{k,h}\frac{1}{2^\secp|\cH|}
% \left\|\bra{k}_{\regR_3}
% (I_{\regC_3}\otimes U_{\regR,\regZ})
% \ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\label{last}.
% \end{align}

% From such $\ket{\tau}$ and $U$, we can construct an adversary $\cA$ that breaks the security of the OWSG as follows:
% \begin{enumerate}
%     \item 
%     Get the $\regR_2$ register of $\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}$ and $\ket{\tau}_\regZ$ as input.
%     \item 
%     Choose $h\gets\cH$. Choose $y\gets \cY$.
%     \item 
%     Apply $I_{\regC_3}\otimes U_{\regR,\regZ}$ on $\ket{h,y}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ$.
%     \item
%     Measure the register $\regR_3$ in the computational basis, and output the result.
% \end{enumerate}
% The probability that $\cA$ outputs $k$ is 
% \begin{align}
% &\sum_{k,h}\frac{1}{2^\secp|\cH|}
% \sum_{y\in \cY}\frac{1}{|\cY|}
% \left\|\bra{k}_{\regR_3}
% (I_{\regC_3}\otimes U_{\regR,\regZ})
% \ket{h,y}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
% &\ge
% \sum_{k,h}\frac{1}{2^\secp|\cH|}
% \frac{1}{2\lfloor 2^r\rfloor}
% \left\|\bra{k}_{\regR_3}
% (I_{\regC_3}\otimes U_{\regR,\regZ})
% \ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
% &\ge\frac{1}{2q\lfloor 2^r\rfloor}.
% \end{align}
% Because
% \begin{align}
% \frac{1}{2q\lfloor 2^r\rfloor}-\frac{1}{2^\delta}
% =\frac{2^\delta-2q\lfloor 2^r\rfloor}{2q2^\delta\lfloor 2^r\rfloor}
% \ge\frac{2^\delta-2q2^r}{2q2^\delta\lfloor 2^r\rfloor}>0,
% \end{align}
% the $\delta$ exponential security of the OWSG is broken.
% Hence the computational binding is shown.

% \paragraph{Statistical hiding.}
% Next we show the statistical hiding.
% Let $\cV$ be the following quantum algorithm.
% \begin{enumerate}
%     \item 
% Get $h$, $h(k)$, and the $\regR_3$ register of $\ket{\Phi_k^{\otimes t}}_{\regR_3,\regC_3}$ as input.
% \item 
% Do the shadow tomography and construct the list of all $k'\in\bit^\secp$ such that
% $\Ver(k',\phi_k)\ge1-\frac{1}{p(\secp)}$.
% \item 
% Compute $h(k')$ for each $k'$ in the list.
% If there is only a single $k^*$ in the list such that $h(k^*)=h(k)$, output $k^*$.
% Otherwise, output $\bot$.
% \end{enumerate}


% Due to the pair-wise independence of $h$,
% \begin{align}
% \Pr_{h\gets\cH}[|G_k\cap h^{-1}(h(k))|=1]
% \ge1-\frac{|G_k|}{|\cY|}
% =1-\frac{|G_k|}{2\lfloor 2^r\rfloor}
% \ge\frac{1}{2}.
% \end{align}
% Hence there exists a unitary $U_\regR$ such that
% \begin{align}
% |\bra{\psi_{1}}(I_\regC\otimes U_\regR)\ket{\psi_{0}}|^2    
% \ge\frac{1}{2}.
% \end{align}
% Due to the Uhlmann's theorem, it means that
% $F(\rho_0,\rho_1)\ge\frac{1}{2}$,
% and therefore $\TD(\rho_0,\rho_1)\le\frac{1}{\sqrt{2}}$.

% In summary, we have constructed $\negl(\secp)$-computationally-binding and $\frac{1}{\sqrt{2}}$-statistically-hiding commitment.
% From the flavor conversion theorem of \cite{EC:HhaMorYam23}, we get
% $\negl(\secp)$-computationally-hiding and $\frac{1}{\sqrt{2}}$-statistically-binding commitment.
% By the parallel repetition, we have
% $\negl(\secp)$-computationally-hiding and $\negl(\secp)$-statistically-binding commitment.
% \end{proof}

% \newpage
% \section{Notes (Giulio)}

% Consider the commitment states are
% \[
% \ket{\mathsf{com}_0} = \sum_{j_1 \dots j_n \in [\lambda]^n} \sum_{h_1\in\mathcal{H}_{j_1}\dots h_n\in\mathcal{H}_{j_n}} \sum_{k_1 \dots k_n} \ket{\{k_i, h_i, h_i(k_i), \Phi_{k_i}^{\otimes t}\}_{i\in[n]},  0 \dots 0}
% \]
% and 
% \[
% \ket{\mathsf{com}_1} = \sum_{j_1 \dots j_n \in [\lambda]^n} \sum_{h_1\in\mathcal{H}_{j_1}\dots h_n\in\mathcal{H}_{j_n}} \sum_{k_1 \dots k_n} \sum_{\kappa \in [n]}\ket{\{k_i, h_i, h_i(k_i), \Phi_{k_i}^{\otimes t}\}_{i\in[n]},  \kappa, k_\kappa}
% \]
% where we will think of:
% \begin{itemize}
%     \item $j_i$ as the guess on the regularity of $k_i$.
%     \item $\mathcal{H}_{j_i}$ as the set of function with image size $2^{j_i}$.
% \end{itemize}
% The idea is that, for a large enough $n$, the state is negl close (in trace distance) from a state supported entirely on vectors where there exists at least one $k_i$ such that the corresponding hash $h_i$ has the correct image size. 

% \paragraph{Statistical Hiding.} For statistical hiding, we can rewrite the above commitment of $1$ as
% \[
% \sum_{j_1 \dots j_n \in [\lambda]^n} \sum_{h_1\in\mathcal{H}_{j_1}\dots h_n\in\mathcal{H}_{j_n}} \sum_{k_1 \dots k_n} \sum_{\kappa \in [n]}\ket{\psi_{j_1 \dots j_n, h_1 \dots h_n, k_1, \dots, k_n},  \kappa, k_\kappa}.
% \]
% Fixing a particular set of values and renormalizing, we obtain
% \[
% \ket{\Psi} = \frac{1}{\sqrt{n}}\sum_{\kappa \in [n]}\ket{\psi_{j_1 \dots j_n, h_1 \dots h_n, k_1, \dots, k_n},  \kappa, k_\kappa}.
% \]
% Say that from any such set we can recover at least one $k_{i^*}$, then we could construct the state
% \[
% \ket{\Psi'} = \ket{\psi_{j_1 \dots j_n, h_1 \dots h_n, k_1, \dots, k_n},  i^*, k_{i^*}}.
% \]
% and note that
% \[
% |\bra{\Psi} \ket{\Psi'}|^2 = 1/n
% \]
% which is noticeable. The general case follows by lower bounding the cross terms of the inner product by $0$. This assumes that the recovery procedure is perfect, but we can account for the cases in which it fails similarly to the above analysis, picking up an additional factor $1/2$ in the fidelity.

% \paragraph{Computational Binding.} For computational binding, I am hoping that we can get away with the reduction guessing the position of such $k_i$. However, at the moment there is a problem: The reduction could decide not to invert the key $k$ that is associated with the ``right'' hash function $h$, and still succeed with inverse-polynomial probability. This breaks the security proof, but I don't think it gives a counterexample against the construction.

% In fact, I think that the unitary $U$ should not be able to succeed only when the hash is picked from the wrong domain. This is because this unitary could be used to estimate the regularity of a randomly sampled key $k$. (One sily idea would be to use this unitary constructive, but this only gives a non-uniform construction)

==> backup_EFI_from_OWSG.tex <==
\section{Exponentially-Secure IV-OWSGs Imply EFIs}
\label{sec:exp_IVOWSG_EFI}
In this section, we show our main result, namely, the construction of EFIs from exponentially-secure IV-OWSGs. 
\mor{the following is wrong if KeyGen is QPT}
Throughout the following section we assume without loss of generality that, for a given $\lambda$, there are \emph{exactly} $2^\lambda$ keys in the support of $\keygen$. This is without loss of generality because we can always treat the random coins $r\in\{0,1\}^\lambda$ of the $\keygen$ algorithm as the ``effective'' key of the IV-OWSG: We can simply define the key generation algorithm to be $r \gets \{0,1\}^\lambda$, then incorporate the $\keygen(1^\lambda; r)$ procedure in both the $\StateGen$ and the $\Ver$ algorithm. This is the same scheme, up to renaming of the algorithms. Before stating our main theorem, we prove a useful lemma below.

\begin{lemma}\label{lem:1}
Let $(\KeyGen,\StateGen,\Ver)$ be a $\delta$-exponentially-secure IV-OWSG. For any polynomial $p=p(\lambda)$ define 
\begin{align*}
G_k\coloneqq \left\{k'\in\KeyGen(1^\secp):\Pr[\top\gets\Ver(k',\phi_k)]\ge 1-\frac{1}{p(\secp)}\right\}.    
\end{align*}
Then 
\[
|G_k|\le 2^r
\]
for any $r$ such that $\delta+r \ge C\secp$, for some constant $C > 1$.
\end{lemma}
\begin{proof}
Consider the following trivial attack against the IV-OWSG: On input $\phi_k^{\otimes t}$, ignore the state, sample $k' \gets \keygen(1^\lambda)$,
and output $k'$. By the $\delta$-exponential security of the IV-OWSG, the winning probability of the trivial attack should be at most $2^{-\delta}$. In other words:
\begin{align*}
\frac{1}{2^{2\secp}}\sum_{k,k'\in\KeyGen(1^\secp)} \Pr[\top\gets\Ver(k',\phi_k)]\le 2^{-\delta}.
\end{align*}
%
Let us define the set of keys 
\begin{align*}
T\coloneqq\{k\in\keygen(1^\secp):|G_k|\ge 2^r\}.    
\end{align*}
Then we rewrite
\begin{align*}
2^{-\delta}
&\ge\frac{1}{2^{2\secp}}\sum_{k,k'\in\KeyGen(1^\secp)} \Pr[\top\gets\Ver(k',\phi_k)]\\
&\ge\frac{1}{2^{2\secp}}\sum_{k\in\KeyGen(1^\secp)} \sum_{k'\in G_k}\Pr[\top\gets\Ver(k',\phi_k)]\\
&\ge\frac{1-\frac{1}{p(\lambda)}}{2^{2\secp}}\sum_{k\in\KeyGen(1^\secp)}|G_k|\\
&\ge\frac{1-\frac{1}{p(\lambda)}}{2^{2\secp}}\sum_{k\in T}|G_k|\\
&\ge\frac{(1-\frac{1}{p(\lambda)})2^r|T|}{2^{2\secp}}.
\end{align*}
Putting things together, we obtain that
\begin{align*}
\frac{|T|}{2^\secp}
\le\frac{2^\secp}{2^{\delta+r}(1-\frac{1}{p(\lambda)})}
\end{align*}
which is negligible if $\delta+r \ge C\secp$, for some $C>1$.
\end{proof}
We are now ready to show the main theorem of this section.
\begin{theorem}\label{thm:EFI_from_IV-OWSG}
Let $\delta\ge (0.5+D)\secp$, for any constant $D>0$. If $\delta$-exponentially secure IV-OWSGs exist, then EFI pairs exist.    
\end{theorem}
\begin{proof}
Let $r\coloneqq(0.5+\frac{D}{2})\secp$ and let $\cH\coloneqq\{h:\cX\to\cY\}$ be the family of pairwise independent hash functions such that $\cX\coloneqq\bit^\secp$ and $\cY\coloneqq\{1,\dots, 2\lfloor 2^r\rfloor\}$. By \cref{cor:com_to_EFI} it suffices to show that IV-OWSGs imply canonical quantum bit commitment schemes that satisfy statistical $(1-1/\poly(\secp))$-hiding and computational binding. 
Assume that an IV-OWSG $(\KeyGen,\StateGen,\Ver)$ exists.
From it, we construct a bit commitment.
We define the following two states, that we shall think of being the commitments of $0$ and $1$, respectively:
\begin{align}
\ket{\psi_{0}}_{\regR,\regC}&\coloneqq
\frac{1}{\sqrt{2^\secp}}
\sum_{k\in\keygen(1^\secp)}
\frac{1}{\sqrt{|\cH|}}
\sum_{h\in\cH}   
\ket{k,h}_{\regC_1}\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\\
\ket{\psi_1}_{\regR,\regC}&\coloneqq
\frac{1}{\sqrt{2^\secp}}
\sum_{k\in\keygen(1^\secp)}
\frac{1}{\sqrt{|\cH|}}
\sum_{h\in\cH}   
\ket{k,h}_{\regC_1}\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{k}_{\regR_3}.
\end{align} 
\mor{Do we assume $\KeyGen$ is just $k\gets\bit^\secp$?}
\takashi{Strictly speaking, we have to give unitaries that generate these states from $\ket{0...0}$ since commitment schemes are defined as a family of unitaries.
Should we mention it? 
}\textcolor{red}{GM: Good idea.}
We denote by $\regC\coloneqq(\regC_1,\regC_2)$ the commitment registers and by $\regR\coloneqq(\regR_1,\regR_2,\regR_3)$ the opening registers.
Without loss of generality, we can assume that $\StateGen$ generates a pure state
$\ket{\Phi_k}_{\regA,\regB}$ and outputs the register $\regA$.
Then, we have $\phi_k=\Tr_{\regB}(\ket{\Phi_k}_{\regA,\regB})$ and consequently we define $\regC_2\coloneqq (\regB_1,...,\regB_t)$
and
$\regR_2\coloneqq (\regA_1,...,\regA_t)$.
It is clear that both $\ket{\psi_0}$ and $\ket{\psi_1}$ are efficiently generatable. %Furthermore, the verification of the commitment is \emph{canonical}, in the sense that the verification simply uncomputes the generating unitary and projects onto $\ket{0\dots 0}\bra{0\dots 0}$. \textcolor{red}{GM: Correct?}\takashi{I think that's part of the definition of binding, and so I don't think we need to state it explicitly.} 
\takashi{I commnted out the following sentence: ``Furthermore, the verification of the commitment is \emph{canonical}, in the sense that the verification simply uncomputes the generating unitary and projects onto $\ket{0\dots 0}\bra{0\dots 0}$." 
This is because there is no concept of ``verification" in the definition of canonical quantum bit commitment. This is implicit in the definition of binding.
}\textcolor{red}{GM: Sounds good.}
In the following we show that the scheme is 
statistical $(1-1/\poly(\secp))$-hiding and computational binding.  
%computationally binding and statistically hiding.



\paragraph{Computational binding.}
Towards a contradiction, we assume that our construction does not satisfy the computational binding.
This means that there exists a polynomial $q=q(\lambda)$, a quantum advice state $\ket{\tau}_\regZ$ on the register $\regZ$,  and
a QPT unitary $U$ acting on $\regR$ and $\regZ$ such that
\begin{align*}
\|\bra{\psi_1}_{\regC,\regR}(I_\regC\otimes U_{\regR,\regZ})(\ket{\psi_0}_{\regC,\regR}\ket{\tau}_\regZ)\|^2\ge\frac{1}{q(\secp)}
\end{align*}
for infinitely-many $\secp$. This means that
\begin{align*}
\frac{1}{q(\secp)}
&\le\left\|
\sum_{k,h}\frac{1}{2^\secp|\cH|} 
\bra{h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
(I_{\regC_2}\otimes U_{\regR,\regZ})
\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
&\le\left(\sum_{k,h}\frac{1}{2^\secp|\cH|} 
\left\|\bra{h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
(I_{\regC_2}\otimes U_{\regR,\regZ})
\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|\right)^2\\
&\le\sum_{k,h}\frac{1}{2^\secp|\cH|} 
\left\|\bra{h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
(I_{\regC_2}\otimes U_{\regR,\regZ})
\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
&\le\sum_{k,h}\frac{1}{2^\secp|\cH|}
\left\|\bra{k}_{\regR_3}
(I_{\regC_2}\otimes U_{\regR,\regZ})
\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\label{last}.
\end{align*}
Here, in the second inequality we have used the triangle inequality, and in the third inequality we have used Jensen's inequality.
From such $\ket{\tau}$ and $U$, we can construct a QPT adversary $\cA$ that breaks the security of the IV-OWSG as follows:
\begin{itemize}
    \item 
    Get the $\regR_2$ register of $\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}$ and $\ket{\tau}_\regZ$ as input.
    \item 
    Choose $h\gets\cH$. Choose $y\gets \cY$.
    \item 
    Apply $(I_{\regC_2}\otimes U_{\regR,\regZ})$ on $\ket{h,y}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ$.
    \item
    Measure the register $\regR_3$ in the computational basis, and output the result.
\end{itemize}
The probability that $\cA$ outputs $k$ is 
\begin{align*}
&\sum_{k,h}\frac{1}{2^\secp|\cH|}
\sum_{y\in \cY}\frac{1}{|\cY|}
\left\|\bra{k}_{\regR_3}
(I_{\regC_3}\otimes U_{\regR,\regZ})
\ket{h,y}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
&\ge
\sum_{k,h}\frac{1}{2^\secp|\cH|}
\frac{1}{2\lfloor 2^r\rfloor}
\left\|\bra{k}_{\regR_3}
(I_{\regC_3}\otimes U_{\regR,\regZ})
\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
&\ge\frac{1}{2q(\lambda)\lfloor 2^r\rfloor}.
\end{align*}
Because
\begin{align*}
\frac{1}{2q(\lambda)\lfloor 2^r\rfloor}-\frac{1}{2^\delta}
=\frac{2^\delta-2q(\lambda)\lfloor 2^r\rfloor}{2q(\lambda)2^\delta\lfloor 2^r\rfloor}
\ge\frac{2^\delta-2q(\lambda)2^r}{2q(\lambda)2^\delta\lfloor 2^r\rfloor}>0,
\end{align*}
$\cA$ breaks the one-wayness of the IV-OWSG with probability $>2^{-\delta}$, which is a contradiction.
Thus, the above scheme satisfies computational binding. 

\paragraph{Statistical hiding.} 
Fix any polynomial $p=p(\secp)$.
Consider the following (inefficient) algorithm that can access only the $\regR$ register of $\ket{\psi_0}_{\regR,\regC}$.
\begin{itemize}
\item Apply the shadow tomography procedure (setting $\varepsilon = 1/p(\lambda)$ and $\omega = 2^{-\lambda}$) 
    on $\regR_2$ register of $\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}$
to obtain the list of all $k'$ such that
$\Ver(k',\phi_k)\ge1-\frac{1}{p(\secp)}$.
\item 
Read $(h,h(k))$ from $\regR_1$.
Compute $h(k')$ for each $k'$ in the list.
If there is only a single $k^*$ in the list such that $h(k^*)=h(k)$, output $k^*$.
Otherwise, output $\bot$.
\end{itemize}
By the pairwise independence of $h$ and by \cref{lem:1}, we have that
\begin{align*}
\Pr_{h\gets\cH}[|G_k\cap h^{-1}(h(k))|=1]
\ge1-\frac{|G_k|}{|\cY|}
=1-\frac{|G_k|}{2\lfloor 2^r\rfloor}
\ge\frac{1}{2}
\end{align*}
except with negligible probability, over the random choice of $k$. 
Setting $t = t(\lambda)$ to be a large enough polynomial, by \cref{lem:ST}, the above inefficient algorithm outputs $k^*$
with probability at least $\frac{1}{2}$.
If we purify the algorithm, we have a unitary $U_\regR$ such that
\begin{align*}
|\bra{\psi_{1}}_{\regR,\regC}(I_\regC\otimes U_\regR)\ket{\psi_{0}}_{\regR,\regC}|^2    
\ge\frac{1}{2}
\end{align*}
\mor{Don't we need ancilla?}
except with negligible probability, over the randomness of the shadow tomography procedure\mor{This is incorporated with the unitary}. By Uhlmann's theorem we have
\[
F(\rho_0,\rho_1)\ge\frac{1}{2} - \negl(\lambda)
\]
where $\rho_b$ denotes the reduced density operator over the $\regC$ register of $\ket{\psi_b}$.
Consequently, $\TD(\rho_0,\rho_1)\le\frac{1}{\sqrt{2}} + \negl(\lambda)$.
This implies that the scheme satisfies 
statistical $(\frac{1}{\sqrt{2}} + \negl(\lambda))$-hiding, which in particular implies that it satisfies statistical $(1-1/\poly(\secp))$-hiding. 
This completes the proof of \Cref{thm:EFI_from_IV-OWSG}. %\takashi{The parallel repetition step is no longer needed since it is already implicitly done in \cref{cor:com_to_EFI}}
\if0
\paragraph{Parallel Repetition.} The above argument shows that there exists a commitment which is computationally binding with negligible probability and $\frac{1}{\sqrt{2}} + \negl(\lambda)$ statistically hiding. The conversion theorem from  \cite{EC:HhaMorYam23} implies that there exists a commitment that is $\negl(\lambda)$ computationally hiding and $\frac{1}{\sqrt{2}} + \negl(\lambda)$ statistically binding. \takashi{I guess there is a quadratic loss in the flavor conversion, and thus this should be $\frac{1}{2^{1/4}} + \negl(\lambda)$ statistically binding. I'll check it and deal with it soon.} By a standard parallel repetition argument, we obtain a commitment which is both statistically binding and computationally hiding with negligible error.
\fi
\end{proof}

%\textcolor{red}{\textbf{GM Marker.}}

% \section{EFI from exponentially-secure mixed OWSGs}
% \takashi{Doesn't this direction work from exponentially-secure IV-OWSGs instead of OWSGs? I don't think the efficient verifiabilility is used in the proof.}
% \begin{definition}[OWSGs] 
% A OWSG is a pair $(\StateGen,\Ver)$ of algorithms such that
% \begin{itemize}
%     \item 
%     $\StateGen(k)\to\phi_k:$
%     It is a QPT algorithm that, on input $k\in\bit^\secp$, outputs an $n$-qubit state $\phi_k$.
%     \item 
%     $\Ver(k',\phi_k)\to\bot/\top:$
%     It is a QPT algorithm that, on input $k'$ and $\phi_k$, outputs $\top/\bot$.
% \end{itemize}
% \end{definition}

% \begin{definition}[Exponential security of OWSGs]
% We say that a OWSG is $\delta$-exponentially-secure if for any QPT adversary $\cA$ and any polynomial $t$,
% \begin{align}
% \Pr[\top\gets\Ver(k',\phi_k):k\gets\bit^\secp,\phi_k^{\otimes t}\gets\StateGen(k)^{\otimes t},k'\gets\cA(1^\secp,\phi_k^{\otimes t})]    
% \le 2^{-\delta}.
% \end{align}
% \end{definition}


% We use the following lemma to show our main result.
% \begin{lemma}
% Let $(\StateGen,\Ver)$ be a $\delta$-exponentially-secure OWSG,  
% $p$ be any polynomial, and
% define
% \begin{align}
% G_k\coloneqq \left\{k'\in\bit^\secp:\Pr[\top\gets\Ver(k',\phi_k)]\ge 1-\frac{1}{p(\secp)}\right\}.    
% \end{align}
% Let $r$ be a polynomial such that
% $\delta+r \ge c\secp$ with a constant $c>1$.
% Then, except for a negligible fraction of $k\in\bit^\secp$, $|G_k|\le 2^r$.
% \end{lemma}
% \begin{proof}
% Let us consider the following trivial attack to the OWSG: given $\phi_k^{\otimes t}$, just ignore it, sample $k'\gets\bit^\secp$, and output $k'$.
% Due to the $\delta$ exponential security of the OWSG, the winning probability of the trivial attack should be at most $2^{-\delta}$:
% \begin{align}
% \frac{1}{2^{2\secp}}\sum_{k,k'\in\bit^\secp} \Pr[\top\gets\Ver(k',\phi_k)]\le2^{-\delta}.
% \end{align}
% Let us define the set
% \begin{align}
% T\coloneqq\{k\in\bit^\secp:|G_k|\ge 2^r\}.    
% \end{align}
% Then,
% \begin{align}
% 2^{-\delta}
% &\ge\frac{1}{2^{2\secp}}\sum_{k,k'\in\bit^\secp} \Pr[\top\gets\Ver(k',\phi_k)]\\
% &\ge\frac{1}{2^{2\secp}}\sum_{k\in\bit^\secp} 
% \sum_{k'\in G_k}\Pr[\top\gets\Ver(k',\phi_k)]\\
% &\ge\frac{1-\frac{1}{p}}{2^{2\secp}}\sum_{k\in\bit^\secp}|G_k|\\
% &\ge\frac{1-\frac{1}{p}}{2^{2\secp}}\sum_{k\in T}|G_k|\\
% &\ge\frac{(1-\frac{1}{p})2^r|T|}{2^{2\secp}}.
% \end{align}
% It means that
% \begin{align}
% \frac{|T|}{2^\secp}
% \le\frac{2^\secp}{2^{\delta+r}(1-\frac{1}{p})}
% \le\negl(\secp)
% \end{align}
% if $\delta+r \ge c\secp$ with $c>1$.
% \end{proof}




% \begin{theorem}
% Let $\delta\ge (0.5+d)\secp$, where $d>0$ is any constant. 
% If $\delta$-exponentially-secure OWSGs exist, then EFI pairs exist.    
% \end{theorem}

% \begin{proof}
% Let $0<\epsilon<1$ be a small constant.
% Let $r\coloneqq(0.5+\frac{d}{2})\secp$.
% Let $\cH\coloneqq\{h:\cX\to\cY\}$ be the family of pairwise independent hash functions such that
% $\cX\coloneqq\bit^\secp$ and $\cY\coloneqq[2\lfloor 2^r\rfloor]$.
% We define the following two states that are used for the commitment of 0 and 1, respectively.
% \begin{align}
% \ket{\psi_{0}}_{\regR,\regC}&\coloneqq
% \frac{1}{\sqrt{2^\secp}}
% \sum_{k\in\bit^\secp}
% \frac{1}{\sqrt{|\cH|}}
% \sum_{h\in\cH}   
% \ket{k,h}_{\regC_1}\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\\
% \ket{\psi_1}_{\regR,\regC}&\coloneqq
% \frac{1}{\sqrt{2^\secp}}
% \sum_{k\in\bit^\secp}
% \frac{1}{\sqrt{|\cH|}}
% \sum_{h\in\cH}   
% \ket{k,h}_{\regC_1}\ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{k}_{\regR_3}.
% \end{align}
% Here, $\regR\coloneqq(\regR_1,\regR_2,\regR_3)$ and $\regC\coloneqq(\regC_1,\regC_2)$.
% Without loss of generality, we can assume that $\StateGen$ runs as follows:
% generate a pure state
% $\ket{\Phi_k}_{\regA,\regB}$ and output the register $\regA$.
% Then, we have $\phi_k=\Tr_{\regB}(\ket{\Phi_k}_{\regA,\regB})$.
% We define $\regC_2\coloneqq (\regB_1,...,\regB_t)$
% and
% $\regR_2\coloneqq (\regA_1,...,\regA_t)$.
% It is clear that both $\ket{\psi_0}$ and $\ket{\psi_1}$ are efficiently generatable.



% \paragraph{Computational binding.}
% First we show the computational binding.
% For the sake of contradiction, we assume that our construction does not satisfy the computational binding.
% It means that there exists a polynomial $q$, a quantum advice state $\ket{\tau}_\regZ$ on the register $\regZ$, and
% a QPT unitary $U$ acting on $\regR$ and $\regZ$ such that
% \begin{align}
% \|\bra{\psi_1}_{\regC,\regR}(I_\regC\otimes U_{\regR,\regZ})(\ket{\psi_0}_{\regC,\regR}\ket{\tau}_\regZ)\|^2\ge\frac{1}{q(\secp)}
% \end{align}
% for infinitely-many $\secp$.
% This means that
% \begin{align}
% \frac{1}{q(\secp)}
% &\le\left\|
% \sum_{k,h}\frac{1}{2^\secp|\cH|} 
% \bra{h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
% (I_{\regC_3}\otimes U_{\regR,\regZ})
% \ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
% &\le\left(\sum_{k,h}\frac{1}{2^\secp|\cH|} 
% \left\|\bra{h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
% (I_{\regC_3}\otimes U_{\regR,\regZ})
% \ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|\right)^2\\
% &\le\sum_{k,h}\frac{1}{2^\secp|\cH|} 
% \left\|\bra{h,h(k)}_{\regR_1}\bra{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\bra{k}_{\regR_3}
% (I_{\regC_3}\otimes U_{\regR,\regZ})
% \ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
% &\le\sum_{k,h}\frac{1}{2^\secp|\cH|}
% \left\|\bra{k}_{\regR_3}
% (I_{\regC_3}\otimes U_{\regR,\regZ})
% \ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\label{last}.
% \end{align}

% From such $\ket{\tau}$ and $U$, we can construct an adversary $\cA$ that breaks the security of the OWSG as follows:
% \begin{enumerate}
%     \item 
%     Get the $\regR_2$ register of $\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}$ and $\ket{\tau}_\regZ$ as input.
%     \item 
%     Choose $h\gets\cH$. Choose $y\gets \cY$.
%     \item 
%     Apply $I_{\regC_3}\otimes U_{\regR,\regZ}$ on $\ket{h,y}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ$.
%     \item
%     Measure the register $\regR_3$ in the computational basis, and output the result.
% \end{enumerate}
% The probability that $\cA$ outputs $k$ is 
% \begin{align}
% &\sum_{k,h}\frac{1}{2^\secp|\cH|}
% \sum_{y\in \cY}\frac{1}{|\cY|}
% \left\|\bra{k}_{\regR_3}
% (I_{\regC_3}\otimes U_{\regR,\regZ})
% \ket{h,y}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
% &\ge
% \sum_{k,h}\frac{1}{2^\secp|\cH|}
% \frac{1}{2\lfloor 2^r\rfloor}
% \left\|\bra{k}_{\regR_3}
% (I_{\regC_3}\otimes U_{\regR,\regZ})
% \ket{h,h(k)}_{\regR_1}\ket{\Phi_k^{\otimes t}}_{\regC_2,\regR_2}\ket{0...0}_{\regR_3}\ket{\tau}_\regZ\right\|^2\\
% &\ge\frac{1}{2q\lfloor 2^r\rfloor}.
% \end{align}
% Because
% \begin{align}
% \frac{1}{2q\lfloor 2^r\rfloor}-\frac{1}{2^\delta}
% =\frac{2^\delta-2q\lfloor 2^r\rfloor}{2q2^\delta\lfloor 2^r\rfloor}
% \ge\frac{2^\delta-2q2^r}{2q2^\delta\lfloor 2^r\rfloor}>0,
% \end{align}
% the $\delta$ exponential security of the OWSG is broken.
% Hence the computational binding is shown.

% \paragraph{Statistical hiding.}
% Next we show the statistical hiding.
% Let $\cV$ be the following quantum algorithm.
% \begin{enumerate}
%     \item 
% Get $h$, $h(k)$, and the $\regR_3$ register of $\ket{\Phi_k^{\otimes t}}_{\regR_3,\regC_3}$ as input.
% \item 
% Do the shadow tomography and construct the list of all $k'\in\bit^\secp$ such that
% $\Ver(k',\phi_k)\ge1-\frac{1}{p(\secp)}$.
% \item 
% Compute $h(k')$ for each $k'$ in the list.
% If there is only a single $k^*$ in the list such that $h(k^*)=h(k)$, output $k^*$.
% Otherwise, output $\bot$.
% \end{enumerate}


% Due to the pair-wise independence of $h$,
% \begin{align}
% \Pr_{h\gets\cH}[|G_k\cap h^{-1}(h(k))|=1]
% \ge1-\frac{|G_k|}{|\cY|}
% =1-\frac{|G_k|}{2\lfloor 2^r\rfloor}
% \ge\frac{1}{2}.
% \end{align}
% Hence there exists a unitary $U_\regR$ such that
% \begin{align}
% |\bra{\psi_{1}}(I_\regC\otimes U_\regR)\ket{\psi_{0}}|^2    
% \ge\frac{1}{2}.
% \end{align}
% Due to the Uhlmann's theorem, it means that
% $F(\rho_0,\rho_1)\ge\frac{1}{2}$,
% and therefore $\TD(\rho_0,\rho_1)\le\frac{1}{\sqrt{2}}$.

% In summary, we have constructed $\negl(\secp)$-computationally-binding and $\frac{1}{\sqrt{2}}$-statistically-hiding commitment.
% From the flavor conversion theorem of \cite{EC:HhaMorYam23}, we get
% $\negl(\secp)$-computationally-hiding and $\frac{1}{\sqrt{2}}$-statistically-binding commitment.
% By the parallel repetition, we have
% $\negl(\secp)$-computationally-hiding and $\negl(\secp)$-statistically-binding commitment.
% \end{proof}

% \newpage
% \section{Notes (Giulio)}

% Consider the commitment states are
% \[
% \ket{\mathsf{com}_0} = \sum_{j_1 \dots j_n \in [\lambda]^n} \sum_{h_1\in\mathcal{H}_{j_1}\dots h_n\in\mathcal{H}_{j_n}} \sum_{k_1 \dots k_n} \ket{\{k_i, h_i, h_i(k_i), \Phi_{k_i}^{\otimes t}\}_{i\in[n]},  0 \dots 0}
% \]
% and 
% \[
% \ket{\mathsf{com}_1} = \sum_{j_1 \dots j_n \in [\lambda]^n} \sum_{h_1\in\mathcal{H}_{j_1}\dots h_n\in\mathcal{H}_{j_n}} \sum_{k_1 \dots k_n} \sum_{\kappa \in [n]}\ket{\{k_i, h_i, h_i(k_i), \Phi_{k_i}^{\otimes t}\}_{i\in[n]},  \kappa, k_\kappa}
% \]
% where we will think of:
% \begin{itemize}
%     \item $j_i$ as the guess on the regularity of $k_i$.
%     \item $\mathcal{H}_{j_i}$ as the set of function with image size $2^{j_i}$.
% \end{itemize}
% The idea is that, for a large enough $n$, the state is negl close (in trace distance) from a state supported entirely on vectors where there exists at least one $k_i$ such that the corresponding hash $h_i$ has the correct image size. 

% \paragraph{Statistical Hiding.} For statistical hiding, we can rewrite the above commitment of $1$ as
% \[
% \sum_{j_1 \dots j_n \in [\lambda]^n} \sum_{h_1\in\mathcal{H}_{j_1}\dots h_n\in\mathcal{H}_{j_n}} \sum_{k_1 \dots k_n} \sum_{\kappa \in [n]}\ket{\psi_{j_1 \dots j_n, h_1 \dots h_n, k_1, \dots, k_n},  \kappa, k_\kappa}.
% \]
% Fixing a particular set of values and renormalizing, we obtain
% \[
% \ket{\Psi} = \frac{1}{\sqrt{n}}\sum_{\kappa \in [n]}\ket{\psi_{j_1 \dots j_n, h_1 \dots h_n, k_1, \dots, k_n},  \kappa, k_\kappa}.
% \]
% Say that from any such set we can recover at least one $k_{i^*}$, then we could construct the state
% \[
% \ket{\Psi'} = \ket{\psi_{j_1 \dots j_n, h_1 \dots h_n, k_1, \dots, k_n},  i^*, k_{i^*}}.
% \]
% and note that
% \[
% |\bra{\Psi} \ket{\Psi'}|^2 = 1/n
% \]
% which is noticeable. The general case follows by lower bounding the cross terms of the inner product by $0$. This assumes that the recovery procedure is perfect, but we can account for the cases in which it fails similarly to the above analysis, picking up an additional factor $1/2$ in the fidelity.

% \paragraph{Computational Binding.} For computational binding, I am hoping that we can get away with the reduction guessing the position of such $k_i$. However, at the moment there is a problem: The reduction could decide not to invert the key $k$ that is associated with the ``right'' hash function $h$, and still succeed with inverse-polynomial probability. This breaks the security proof, but I don't think it gives a counterexample against the construction.

% In fact, I think that the unitary $U$ should not be able to succeed only when the hash is picked from the wrong domain. This is because this unitary could be used to estimate the regularity of a randomly sampled key $k$. (One sily idea would be to use this unitary constructive, but this only gives a non-uniform construction)
